ModuLoRA: Finetuning 2-Bit LLMs on Consumer GPUs by Integrating with Modular Quantizers

We propose a memory-efficient finetuning algorithm for large language models (LLMs) that supports finetuning LLMs with 65B parameters in 2/3/4-bit precision on as little as one 24GB GPU. Our method, modular low-rank adaptation (ModuLoRA), integrates any user-specified weight quantizer with finetuning via low-rank adapters (LoRAs). Our approach relies on a simple quantization-agnostic backward pass that adaptively materializes low-precision LLM weights from a custom black-box quantization module. This approach enables finetuning 2-bit and 3-bit LLMs for the first time -- leveraging state-of-the-art 2-bit QuIP\# quantization and 3-bit OPTQ quantization -- outperforming finetuning that relies on less sophisticated 4-bit and 8-bit methods. In our experiments, \lplora~attains competitive performance on text classification, natural language inference, and instruction following tasks using significantly less memory than existing approaches, and we also surpass the state-of-the-art ROUGE score on a popular summarization task. We release \lplora~together with a series of low-precision models as part of \llmtune, a user-friendly library for quantizing, running, and finetuning LLMs on consumer GPUs.

==> figs/memory_requirements_combined.tex <==
\begin{figure}[ht]
    \begin{minipage}[b]{0.5\linewidth}
        \centering
        \begin{adjustbox}{max width=\textwidth}
            \begin{tabular}{l@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c}
                \toprule[1.3pt]
                LLaMA Finetuning & 7B & 13B & 30B & 65B \\
                \midrule
                \llmtune~(3-bit) &  5.5 GB  & 9.3 GB  & 19.4 GB & 35.4 GB \\
                \llmtune~(4-bit) & 5.0 GB & 8.8 GB  & 20.4 GB & 38.8 GB \\
                \midrule
                Full Precision & 38.0 GB & 73.9 GB  & 183.3 GB  & 360.4 GB \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
        \captionof{table}{Memory requirements}
        \label{tab:memory_requirements_table}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.5\linewidth}
        \centering
\begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}] 
\begin{axis}[
	axis lines = left, % Connect the y-axis with the x-axis at the bottom
	xlabel = {Model Parameter Size (Billion)},
	ylabel = {Required Memory (Gigabyte)},
	xmin=0, xmax=70, % Adjusted for the B units
	ymode=log, % Set y-axis to logarithmic scale
	log basis y={10}, % Logarithm base 10
	log ticks with fixed point, % Display labels in fixed point notation
	ymin=1, % Set the minimum y value close to zero that can be represented on a log scale
	ymax=400, % Adjusted to include the highest y-value
	xtick={7,13,33,65},
	xticklabels={7B,13B,33B,65B},
	ytick={1,10,100,400},
	yticklabels={0GB,10GB,100GB,400GB}, % Manually set the label of the first tick to "0"
	legend style={at={(0.98,0.02)}, anchor=south east}, % Move the legend inside the plot to the bottom right
	ymajorgrids=true,
	grid style=dashed,
	every node near coord/.append style={font=\small}, % Make the font size of nodes near coords slightly bigger
]

% Data from the table for 3bit with labels
\addplot[
    color=teal,
    mark=square,
    nodes near coords,
    point meta=explicit symbolic,
    every node near coord/.append style={yshift=1.5mm}, % Shift nodes for 3bit up a bit
    ]
    coordinates {
    (7,5.5) [5.5]
    (13,9.3) [9.3]
    (33,19.4) [19.4]
    (65,35.4) [35.4]
    };
\addlegendentry{LLMTools (3-bit)}

% Data from the table for 4bit
\addplot[
    color=cyan,
    mark=o,
    ]
    coordinates {
    (7,5)(13,8.8)(33,20.4)(65,38.8)
    };
\addlegendentry{LLMTools (4-bit)}

% Data from the table for Full precision with labels
\addplot[
    color=darkgray,
    mark=star,
    nodes near coords,
    point meta=explicit symbolic,
    ]
    coordinates {
    (7,38) [38]
    (13,73.9) [73.9]
    (33,183.3) [183.3]
    (65,360.4) [360.4]
    };
\addlegendentry{Full precision}

% Dotted line showing the difference between Full precision and 3bit
\draw [dotted, thick] (axis cs:7,5.2) -- (axis cs:7,38);
\draw [dotted, thick] (axis cs:13,9.3) -- (axis cs:13,73.9);
\draw [dotted, thick] (axis cs:33,19.4) -- (axis cs:33,183.3);
\draw [dotted, thick] (axis cs:65,35.4) -- (axis cs:65,360.4);

% Dotted line showing the difference between Full precision and 3bit
\draw [dotted, thick] (axis cs:7,5.2) -- (axis cs:7,3);
\draw [dotted, thick] (axis cs:13,9.3) -- (axis cs:13,73.9);
\draw [dotted, thick] (axis cs:33,19.4) -- (axis cs:33,183.3);
\draw [dotted, thick] (axis cs:65,35.4) -- (axis cs:65,360.4);

\end{axis}
\end{tikzpicture}
        \caption{Memory requirements for different precision models.}
        \label{fig:memory_requirements_combined}
    \end{minipage}
\end{figure}


==> tables/app_02_defense_agg.tex <==
\begin{table*}
\centering
\begin{tabular}{lrr}
\toprule
$\lambda$ & NDCG@10 & BLEU \\
\midrule
0.000 & 0.302 & 80.372 \\
0.001 & 0.302 & 72.347 \\
0.010 & 0.296 & 10.334 \\
0.100 & 0.002 & 0.148 \\
1.000 & 0.001 & 0.080 \\
\bottomrule
\end{tabular}
\label{app:tab:defense_aggregate_results}
\caption{Retrieval performance and reconstruction performance across varying noise levels $\lambda$.}
\end{table*}

==> tables/bbh.tex <==
\begin{wraptable}{r}{9cm}
\centering
% \vspace{-5mm}
\vspace{-40pt}
{
    \begin{tabular}{l@{\hskip 0.3in}c@{\hskip 0.3in}c@{\hskip 0.3in}c@{\hskip 0.3in}c}
    \toprule
    Baseline Scores & L & XL & XXL & {\small PALM} \\
    \midrule
    { FLaN/PALM (32-bit)} & 30.3 & 39.9  & 47.4  & 37.4 \\
    \bottomrule
    \toprule
     Alpaca Scores & 7B & 13B & 30B & 65B \\
    \midrule
    { \llmtune~(3-bit)} & 31.1  & 35.3   & 37.2 & 43.3 \\
    { \llmtune~(4-bit)} & 33.1 & 36.2 & 40.4 & 43.7 \\
    { Bits\&Bytes~(4-bit)} & 31.9 & 35.4 & 39.0 & 45.1 \\
    { Bits\&Bytes~(8-bit)} & 33.3 & 36.8 & 39.1 & 46.1 \\
    { Bits\&Bytes~(16-bit)} & 33.7 & 37.1 & 41.3 & 46.8 \\
    \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \captionof{table}{Instruction-tuned models evaluated on BigBench Hard (BBH). We finetune LLaMA models on the Alpaca dataset in 3 to 16 bits. The results have a variation of around $\pm0.5$.}
    \label{tab:bbh}
    \vspace{-60pt}
}
\end{wraptable}
% }
% \captionof{table}{Instruction-tuned models evaluated on BigBench Hard (BBH). We finetune LLAMA models on the Alpaca dataset in 3 to 16 bits. The results have a variation of around $\pm0.5$.}
% \label{tab:bbh}
% \vspace{-4mm}
% \end{table}

==> tables/opt.tex <==
\begin{table}[t]
    \centering
% \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc}
    \toprule
     OPT Finetuning & 7B & 13B \\
    \midrule
    \llmtune~(4-bit) & - & - \\
    Bits\&Bytes~(8-bit) & - & - \\
    \bottomrule
    \end{tabular}
% }
\caption{Round-to-Nearest Quantization.}
\label{tab:rtn}
\end{table}
